Situation Awareness for Driver-Centric Driving Style Adaptation

There is evidence that the driving style of an autonomous vehicle is important to increase the acceptance and trust of the passengers. The driving situation has been found to have a significant influence on human driving behavior. However, current driving style models only partially incorporate driving environment information, limiting the alignment between an agent and the given situation. Therefore, we propose a situation-aware driving style model based on different visual feature encoders pretrained on fleet data, as well as driving behavior predictors, which are adapted to the driving style of a specific driver. Our experiments show that the proposed method outperforms static driving styles significantly and forms plausible situation clusters. Furthermore, we found that feature encoders pretrained on our dataset lead to more precise driving behavior modeling. In contrast, feature encoders pretrained supervised and unsupervised on different data sources lead to more specific situation clusters, which can be utilized to constrain and control the driving style adaptation for specific situations. Moreover, in a real-world setting, where driving style adaptation is happening iteratively, we found the MLP-based behavior predictors achieve good performance initially but suffer from catastrophic forgetting. In contrast, behavior predictors based on situationdependent statistics can learn iteratively from continuous data streams by design. Overall, our experiments show that important information for driving behavior prediction is contained within the visual feature encoder. The dataset is publicly available at huggingface.co/datasets/jHaselberger/SADC-Situation-Awareness-for-Driver-Centric-Driving-Style-Adaptation.

==> sections/acknowledgment.tex <==
\section*{Acknowledgment}
The authors would like to thank...

==> sections/driver-centric_driving_style_adaptation.tex <==
\section{Driver-Centric Driving Style Adaptation}
\begin{itemize}
    \item Every driver has own driving style
    \item Situation awareness of human like driving
    \item personalization/adaption necessary for user trust ...
    \item fast leraning of personalized driving style
    \item limited data available for vast amount of possible situations
    \item avoid catastrophic forgetting
\end{itemize}

\subsection{Method}
\begin{itemize}
    \item driver specific datasets with unseen roads
    \item How to adapt  
\end{itemize}

\subsection{Experiments}
\begin{itemize}
    \item Effects on the pretrain dataset and on the drivers' test data
    \item training time and complexity needed
    \item plots time series of LUT and MLP approach, highlight cluster centroids
\end{itemize}



==> sections/unsupervised_situation_awareness.tex <==
\section{Unsupervised Situation Awareness}
\label{sec:unsupervised_situation_awareness}

\begin{itemize}
    \item Scalability
    \item basic advantages of unsupervised learning
    \item robustness of the embeddings and found clusters
\end{itemize}

\subsection{Method}
\begin{itemize}
    \item model selection
    \item pretrained or fine-tuned on driving data
    \item freeze 
    \item train MLP head on frozen feature extractor
\end{itemize}

\subsection{Experiments}
\begin{itemize}
    \item visual comparison of found clusters
    \item eval number of clusters
    \item eval catastrophic forgetting
    \item Effects on the pretrain dataset and on the drivers' test data
\end{itemize}
